Recurrent Predictive State Policy Networks

We introduce Recurrent Predictive State Policy (RPSP) networks, a recurrent architecture that brings insights from predictive state representations to reinforcement learning in partially observable environments. Predictive state policy networks consist of a recursive filter, which keeps track of a belief about the state of the environment, and a reactive policy that directly maps beliefs to actions, to maximize the cumulative reward. The recursive filter leverages predictive state representations (PSRs) (Rosencrantz and Gordon, 2004; Sun et al., 2016) by modeling predictive state-- a prediction of the distribution of future observations conditioned on history and future actions. This representation gives rise to a rich class of statistically consistent algorithms (Hefny et al., 2018) to initialize the recursive filter. Predictive state serves as an equivalent representation of a belief state. Therefore, the policy component of the RPSP-network can be purely reactive, simplifying training while still allowing optimal behaviour. Moreover, we use the PSR interpretation during training as well, by incorporating prediction error in the loss function. The entire network (recursive filter and reactive policy) is still differentiable and can be trained using gradient based methods. We optimize our policy using a combination of policy gradient based on rewards (Williams, 1992) and gradient descent based on prediction error. We show the efficacy of RPSP-networks under partial observability on a set of robotic control tasks from OpenAI Gym. We empirically show that RPSP-networks perform well compared with memory-preserving networks such as GRUs, as well as finite memory models, being the overall best performing method.

==> Experiments-Exp2.tex <==
% !TEX root = main.tex
\subsection{Training Time}
\label{sec:exp2}



==> RNNconnection.tex <==
% !TEX root = main.tex
\subsection{Predictive States vs. hidden states LSTMs}
\label{sec:rnnconnection}

In many realistic RL tasks, such as those in robotics and manipulation it is vital to consider incomplete or partial observability. In this setting, models with a hidden-state structure play a crucial role. They provide enough representational power to account for this uncertainty.
Furthermore more complex processes, are often non-Markovian, which require models to keep an internal memory of previous observations. Recurrent neural networks (RNNs) appear to be a common approach to track memory through its internal representation~\cite{WierstraRPG}. Combined with long-short-term memories (LSTMs) they improve the myopic behaviour of vanilla RNNs and allow for more long term dependencies~\cite{Ballesteros16}. 
In this work, we propose an alternative representation of internal state that can leverage internal memory with additional benefits, via a predictive state representation $q_t$. We consider an RNN where the internal state is defined as the expectation of sufficient future statistics condition on all previous observations. This internal structure comprises both a memory component together with a predictive element.
In this sense predictive states track all necessary past information that is sufficient to predict future observations. \\
The training mechanism of learning predictive states bares many similarities with that of training hidden states. In both cases the state is updated via a series of alternate linear and a non-linear transformations. For predictive states $p_t$ the linear transformation $W_{sys}p_t$ represents the system prediction: from expectations over futures $p_t$ to expectations over extended features $q_t$. The non-linear transformation, $F_t$ is a filtering function that conditions on the current action and observation to update the expectation of the consecutive future statistics $q_{t+1}$, in \eref{eq:filtering}, in place of the usual activation functions (tanh, relu).
In this paper we initialize these weights, using a moment matching technique, with good theoretical guarantees, \sref{sec:psr}.


%PSRs also define computation graphs
%advantage of using policy learning with predictive states
%update the policy parameter by leveraging the states of the system
%states both keep making good predictions and fully describe the system have memory they learn to track in RKHS space the distribution of future observations based on past histories 
%can leverage history like LSTM with additional benefit of b


==> Training-CrossEntropy.tex <==
% !TEX root = main.tex
\subsection{Cross Entropy with Predictive States}
\label{sec:crossentropy}



